On Symbolically Encoding the Behavior of Random Forests

Recent work has shown that the input-output behavior of some machine learning systems can be captured symbolically using Boolean expressions or tractable Boolean circuits, which facilitates reasoning about the behavior of these systems. While most of the focus has been on systems with Boolean inputs and outputs, we address systems with discrete inputs and outputs, including ones with discretized continuous variables as in systems based on decision trees. We also focus on the suitability of encodings for computing prime implicants, which have recently played a central role in explaining the decisions of machine learning systems. We show some key distinctions with encodings for satisfiability, and propose an encoding that is sound and complete for the given task.

==> figs/dt-tikz.tex <==

\tikzset{
  treenode/.style = {align=center, inner sep=0pt, text centered,
    font=\sffamily},
  arn/.style = {treenode, circle, black, font=\sffamily\bfseries, draw=black, text width=5em},
  arn_leaf/.style = {treenode, circle, draw=black, text width=3em}
}

\begin{figure}[t]
\centering
\begin{tikzpicture}[->,>=stealth',level/.style={sibling distance = 5cm/#1,
  level distance = 2cm}] 
\node [arn] {\(X \geq 2\)}
    child{ node [arn] {\(Y \geq -7\)} 
            child{ node [arn_leaf] {0} }
            child{ node [arn_leaf] {1} }                     
    }
    child{ node [arn] {\(X \geq 6\)}
            child{ node [arn_leaf] {1} }
            child{ node [arn_leaf] {0} }
		}
; 
\end{tikzpicture}
\caption { A decision tree on continuous variables \(X\) and \(Y\). Right branch means test is true, left branch means test is false. \label{fig:dt}}
\end{figure}


==> figs/dt-tikz2.tex <==

\tikzset{
  treenode/.style = {align=center, inner sep=0pt, text centered,
    font=\sffamily},
  arn/.style = {treenode, circle, black, font=\sffamily\bfseries, draw=black, text width=5em},
  arn_leaf/.style = {treenode, circle, draw=black, text width=3em}
}

\begin{figure}[t]
\centering
\begin{minipage}[]{.6\textwidth}
\centering
\scalebox{.8}[.8]{
\begin{tikzpicture}[->,>=stealth',level/.style={sibling distance = 5cm/#1,
  level distance = 2cm}] 
\node [arn] {\(X \geq 2\)}
    child{ node [arn] {\(Y \geq -7\)} 
            child{ node [arn_leaf] {0} }
            child{ node [arn_leaf] {1} }                     
    }
    child{ node [arn] {\(X \geq 6\)}
            child{ node [arn_leaf] {1} }
            child{ node [arn_leaf] {0} }
		}
; 
\end{tikzpicture}
}
\end{minipage}
\begin{minipage}[]{.35\textwidth}
    \centering
    \begin{tabular}{c|c} 
    Discrete Value & Interval \\ \hline
    \(x_1\) & \((-\infty, 2)\) \\
     \(x_2\) & \([2, 6)\) \\
     \(x_3\) & \([6,+\infty)\) \\ \hline
     \(y_1\) & \((-\infty, -7)\) \\
     \(y_2\) & \([-7,+\infty)\) \\
    \end{tabular}\\
    \bigskip
    \begin{tabular}{cc|c}
        \(X\)           & \(Y\)             & \(f(X,Y)\)    \\
        \hline
        
        \(x_1\)  & \(y_1\)      & 0 \\
        \(x_1\)  & \(y_2\)      & 1 \\
        
        \(x_2\)        & \(y_1\)       & 1 \\
        \(x_2\)        & \(y_2\)       & 1 \\
        
        \(x_3\)   & \(y_1\)      & 0 \\
        \(x_3\)   & \(y_2\)      & 0 \\
    \end{tabular}
\end{minipage}
\caption {(Left) A decision tree on continuous variables \(X\) and \(Y\). Right branch means test is true, left branch means test is false. (Right) The discrete function represented by the decision tree. \label{fig:dt}}
\end{figure}


==> stdmacros.tex <==
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem{definition}{Definition}
%\newtheorem{proposition}{Proposition}


\def\definedas{{\:\:\stackrel{\it def}{=}\:\:}}
\newcommand\shrink[1]{}
\newcommand{\art}[1]{{\color{red} \textit{[Art: #1~]}}}
\def\n(#1){\bar{#1}}
\def\bn{{\mathcal{N}}}
\def\data{\mathcal{D}}
\def\pr{{\it Pr}}
\def\prp{{\it Pr^\prime}}
\def\A{{\bf A}}
\def\a{{\bf a}}
\def\B{{\bf B}}
\def\b{{\bf b}}
\def\C{{\bf C}}
\def\c{{\bf c}}
\def\D{{\bf D}}
\def\E{{\bf E}}
\def\e{{\bf e}}
\def\Pa{{\bf P}}
\def\pa{{\bf p}}
\def\p{{\bf p}}
\def\N{{\bf N}}
\def\T{{\bf T}}
\def\U{{\bf U}}
\def\u{{\bf u}}
\def\V{{\bf V}}
\def\v{{\bf v}}
\def\T{{\bf T}}
\def\W{{\bf W}}
\def\w{{\bf w}}
\def\X{{\bf X}}
\def\x{{\bf x}}
\def\Y{{\bf Y}}
\def\y{{\bf y}}
\def\Z{{\bf Z}}
\def\z{{\bf z}}
\def\sbn{\mathcal{B}}
\def\networkpoly{\mathcal{F}}
\def\ClusterDAG{\mathcal{B}}
\def\eql(#1,#2){{#1\!\!=\!#2}}

\def\eql(#1,#2){{#1\!=\!#2}}
\newcommand\name[1]{\ensuremath{\mathsf{#1}}}
\def\true{\name{true}}
\def\false{\name{false}}

\newcommand{\argmax}{\operatornamewithlimits{arg max}}
\newcommand{\argmin}{\operatornamewithlimits{arg min}}
\newcommand\underbracetxt[2]{\underbrace{{#1}}_{\text{{#2}}}}

%\newenvironment{proofnobox}[1][Proof]
%			   {\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}
%			   {\end{trivlist}}

% math version of smash,llap,rlap by Alexander R. Perlis
\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathrlap{\mathpalette\mathrlapinternal}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathllapinternal#1#2{%
  \llap{$\mathsurround=0pt#1{#2}$}}
\def\mathrlapinternal#1#2{%
  \rlap{$\mathsurround=0pt#1{#2}$}}
\def\mathclapinternal#1#2{%
  \clap{$\mathsurround=0pt#1{#2}$}}

\newcommand\Amain[1]{
\textbf{main:}
#1
\vspace{1mm}
}

\newcommand\Aglobal[1]{
\vspace{1mm}
\textbf{global:} #1
}

\newcommand\Aglobala[2]{
{\bf global:}\\
\begin{tabular}{ll}
#1: & #2
\end{tabular}
}

\newcommand\Anotes[1]{
{\bf notes:}
#1
\vspace{1mm}
}

\newcommand\Ainput[1]{
\vspace{1mm}
\textbf{input:} #1
}

\newcommand\Ainputa[2]{
{\bf input:}\\
\begin{tabular}{ll}
#1: & #2
\end{tabular}
}

\newcommand\Ainputb[4]{
\vspace{1mm}
\textbf{input:}\\
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1}
\begin{tabular}{ll}
#1: & #2 \\
#3: & #4
\end{tabular}
}

\newcommand\Ainputc[6]{
\vspace{1mm}
\textbf{input:}\\
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1}
\begin{tabular}{ll}
#1: & #2 \\
#3: & #4 \\
#5: & #6
\end{tabular}
}

\newcommand\Ainputd[8]{
\vspace{1mm}
\textbf{input:}\\
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1}
\begin{tabular}{ll}
#1: & #2 \\
#3: & #4 \\
#5: & #6 \\
#7: & #8
\end{tabular}
}

\newcommand\Aoutput[1]{
\vspace{1mm}
\textbf{output:} #1
\vspace{1mm}
}

\newcommand\Asupport[1]{
{\bf supporting functions:}
#1
\vspace{1mm}
}

